HeTM: Transactional Memory for Heterogeneous Systems

Modern heterogeneous computing architectures, which couple multi-core CPUs with discrete many-core GPUs (or other specialized hardware accelerators), enable unprecedented peak performance and energy efficiency levels. Unfortunately, though, developing applications that can take full advantage of the potential of heterogeneous systems is a notoriously hard task. This work takes a step towards reducing the complexity of programming heterogeneous systems by introducing the abstraction of Heterogeneous Transactional Memory (HeTM). HeTM provides programmers with the illusion of a single memory region, shared among the CPUs and the (discrete) GPU(s) of a heterogeneous system, with support for atomic transactions. Besides introducing the abstract semantics and programming model of HeTM, we present the design and evaluation of a concrete implementation of the proposed abstraction, which we named Speculative HeTM (SHeTM). SHeTM makes use of a novel design that leverages on speculative techniques and aims at hiding the inherently large communication latency between CPUs and discrete GPUs and at minimizing inter-device synchronization overhead. SHeTM is based on a modular and extensible design that allows for easily integrating alternative TM implementations on the CPU's and GPU's sides, which allows the flexibility to adopt, on either side, the TM implementation (e.g., in hardware or software) that best fits the applications' workload and the architectural characteristics of the processing unit. We demonstrate the efficiency of the SHeTM via an extensive quantitative study based both on synthetic benchmarks and on a porting of a popular object caching system.

==> sections/2_1_demonstration.tex <==
\section*{Appendix: Proof of Correctness}
\label{sec:rs_ws_dem}
\label{sec:rs_ws_proof_appendix}

\hetm enables TM on heterogeneous systems (CPU plus discrete-GPU). However, given the high cost of inter-device communication, \hetm does not track conflicts on a fine-grained fashion. Instead, conflicts are tracked on a batch size granularity, relies on existing TM for the different devices to managed intra-device conflicts and collect the corresponding write-/read-set.

This approach minimizes memory transfers. Because previous works identified that, in general, transactional workloads tend to be read-intensive~\cite{palmieri10}, an efficient design relies on transferring the write-set of transactions, keeping the read-sets locally in the device, performing local comparisons with the transferred, relatively small, write-set.

Figure~\ref{fig:hetm_ws_intersect} presents a case where both devices can commit successfully, i.e., the GPU does not read from the CPU write-set. 

% HeTM_WS_intersect
\hetm compares the $\text{RS}^\text{GPU}$ with the transferred $\text{WS}^\text{CPU}$. As GPU transactions are serialized after the CPU ones.

\hetm compares the read-set in the GPU ($\text{RS}^\text{GPU}$) with the transferred write-set of the CPU ($\text{WS}^\text{CPU}$). If both executions are compatible, i.e., they do not conflict ($\text{RS}^\text{GPU} \cap \text{WS}^\text{CPU} = \emptyset$), then they can be safely merged. Note that this is only possible on the assumption of ``no blind writes'' (i.e., $\text{WS}^\text{GPU} \subseteq \text{RS}^\text{GPU}$ and $\text{WS}^\text{CPU} \subseteq \text{RS}^\text{CPU}$), where we can derive that, if the $\text{RS}^\text{GPU}$ does not intersect $\text{WS}^\text{CPU}$, then, also the $\text{WS}^\text{GPU}$ does not intersect $\text{WS}^\text{CPU}$, i.e.,

$$
\text{RS}^\text{GPU} \cap \text{WS}^\text{CPU} = \emptyset \xrightarrow{\text{WS}^\text{GPU} \subseteq \text{RS}^\text{GPU}} \text{WS}^\text{GPU} \cap \text{WS}^\text{CPU} = \emptyset
$$

This approach does not guarantee that $\text{WS}^\text{GPU}$ does not intersect $\text{RS}^\text{CPU}$, i.e., the CPU may read values produced by the GPU, as shown in Figure~\ref{fig:hetm_ws_intersect}. For this reason \hetm serializes GPU transactions after CPU ones, i.e.,

$$
	\text{CPU} \xrightarrow{\text{serializes before}} \text{GPU}
$$

\begin{figure}[tbp]
	\centering
	\includegraphics[width=0.75\columnwidth]{HeTM_WS_intersect}
	\caption{Comparing the $\text{RS}^\text{GPU}$ with the transferred $\text{WS}^\text{CPU}$.}
	\label{fig:hetm_ws_intersect}
\end{figure}


==> sections/figures.tex <==

% Make sure all figures on single page
% \afterpage{\clearpage}
% \clearpage

\begin{figure}[tbp]
	\centering
	\includegraphics[width=0.99\columnwidth]{batch_size_gpu}
	\caption{Transaction batch size in Array benchmark.}
	\label{fig:batch_size}
\end{figure}

\begin{figure}[tbp]
	\centering
	\includegraphics[width=0.99\columnwidth]{instrumentation_cost}
	\caption{Instrumenting transaction sets in Array benchmark.}
	\label{fig:instrCost}
\end{figure}

\begin{figure}[tbp]
	\centering
	\includegraphics[width=0.99\columnwidth]{array_inter_conflicts}
	\caption{Inter-device conflicts in Array benchmark.}
	\label{fig:interConfl}
\end{figure}

\begin{figure}[tbp]
	\centering
	\includegraphics[width=0.99\columnwidth]{array_prec_writes}
	% \vspace{10pt}
	\includegraphics[width=0.99\columnwidth]{array_time_bars}
	\includegraphics[width=0.99\columnwidth]{array_copy_bars}
	\caption{Synchronizing CPU and GPU in Array benchmark.}
	\label{fig:hetm_vs_theo}
\end{figure}

%% Memcached Benchmark

\begin{figure}[tbp]
	\centering
	%\includegraphics[width=0.99\columnwidth]{__PLOT__HeTM_vs_device_0}
	\caption{Throughput of HeTM for Memcached with fully partitionable workload.}
	\label{fig:memcd-1}
\end{figure}

% \clearpage

\begin{figure}[tbp]
	\centering
	%\includegraphics[width=0.99\columnwidth]{__PLOT__HeTM_vs_device_1a}
	\caption{Throughput of HeTM for Memcached idling one processing unit.}
	\label{fig:memcd-2}
\end{figure}

\begin{figure}[tbp]
	\centering
	%\includegraphics[width=0.99\columnwidth]{__PLOT__HeTM_vs_device_1b}
	\caption{Throughput of HeTM for Memcached with possible conflicts.}
	\label{fig:memcd-3}
\end{figure}


==> sections/title_acm.tex <==
\title{HeTM: Transactional Memory for \\Heterogeneous Systems}

\iftrue % Double blind % ACM Template Format
% Submissions (both abstract and paper) should be prepared for double-blind review, i.e., without author names or other identifying material. Authors should refer to themselves in the third person when citing their own work. 

\usepackage[symbol]{footmisc}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\author{Daniel Castro}
\affiliation{\small%
  % \institution{INESC-ID \& Instituto Superior T{\'e}cnico}
  \department{INESC-ID. Instituto Superior T\'{e}cnico}
  \institution{Universidade de Lisboa}
  \city{Lisbon}
  \country{Portugal}
}
% \email{daniel.castro@ist.utl.pt}
\email{daniel.castro@tecnico.ulisboa.pt}

% \author{Ricardo Vieira}
% \affiliation{%
%   \department{Instituto Superior T{\'e}cnico}
%   \institution{Universidade de Lisboa}
%   \city{Lisbon}
%   \country{Portugal}
% }
% \email{ricardo.vieira@tecnico.ulisboa.pt}

\author{Aleksandar Ilic}
\affiliation{\small%
  \department{INESC-ID. Instituto Superior T\'{e}cnico}
  \institution{Universidade de Lisboa}
  \city{Lisbon}
  \country{Portugal}
}
\email{aleksandar.ilic@tecnico.ulisboa.pt}

\author{Paolo Romano}
\affiliation{\small%
  \department{INESC-ID. Instituto Superior T\'{e}cnico}
  \institution{Universidade de Lisboa}
  \city{Lisbon}
  \country{Portugal}
}
\email{romanop@gsd.inesc-id.pt}

\author{Amin M. Khan}
\affiliation{\small%
  \department{Department of Computer Science}
  \institution{UiT The Arctic University of Norway}
  \city{Troms\o}
  \country{Norway}
}
\email{amin.khan@uit.no}
\fi % Double blind

\renewcommand{\shortauthors}{D. Castro et al.}
% \renewcommand{\shortauthors}{Authors et al.}
